Are Mutually Intelligible Languages Easier to Translate?

Two languages are considered mutually intelligible if their native speakers can communicate with each other, while using their own mother tongue. How does the fact that humans perceive a language pair as mutually intelligible affect the ability to learn a translation model between them? We hypothesize that the amount of data needed to train a neural ma-chine translation model is anti-proportional to the languages' mutual intelligibility. Experiments on the Romance language group reveal that there is indeed strong correlation between the area under a model's learning curve and mutual intelligibility scores obtained by studying human speakers.

==> BAK_04_results.tex <==
\section{Results}

\omer{We will probably remove all of this section}

\subsection{Romance}

Table \ref{table:auc_romance} shows the area under curve (AUC) for each language pair. By looking at the area under curve, we gain a quantifiable insight in to the performance of the machine on a given language pair. The highest AUC score is given to the language pair of highest mutual intelligibility, Italian - Spanish. The correlation between relative BLEU scores and mutual intelligibility score is not significant (Pearson's r = 0.43, p-value = 0.16)

Figure \ref{fig:average_romance} shows the increasing average relative BLEU score of two groups: those who are considered to be of high and low intelligibility. It can be seen that the high intelligibility group achieves higher relative BLEU scores at the start of the process. Table \ref{table:romance1} shows the raw BLEU results on the test set, for the Roman  languages, for all data sizes.

Some language pairs are congruent with our hypothesis, for example, Figure \ref{fig:romance_cherry} shows the relative BLEU score in each subset of the data for two pairs of languages- Italian Spanish and Spanish-Romanian. It can be seen that the Spanish - Italian pair reaches a level close to saturation after using only 70\% of the data, which is consistent with their high intelligibility, as opposed to Spanish - Romanian, which saturates at 80\% of the data. We define saturation point as percentage of data which surpasses the 0.95 relative BLEU score


\begin{table*}[t]
\small
\centering
\begin{tabular}{
>{\columncolor[HTML]{EFEFEF}}l l}
{\color[HTML]{000000} ES FR} & 73.632 \\
{\color[HTML]{000000} \textbf{ES IT}} & 73.742 \\
{\color[HTML]{000000} \textbf{RO FR}} & 70.478 \\
{\color[HTML]{000000} \textbf{RO ES}} & 71.871 \\
{\color[HTML]{000000} \textbf{RO IT}} & 71.477 \\
{\color[HTML]{000000} \textbf{IT ES}} & 74.342 \\
{\color[HTML]{000000} \textbf{IT FR}} & 72.688 \\
{\color[HTML]{000000} ES RO} & 71.766 \\
{\color[HTML]{000000} FR IT} & 72.543 \\
{\color[HTML]{000000} FR ES} & 72.891 \\
{\color[HTML]{000000} FR RO} & 69.939 \\
{\color[HTML]{000000} IT RO} & 71.714
\end{tabular}
\caption{AUC score per Romance language pair. In each row, first language is source and last language is destination. Marked in bold are language pairs which are of high intelligibility.}
\label{table:auc_romance}
\end{table*}

\begin{table*}[t]
\small
\centering
\begin{tabular}{
>{\columncolor[HTML]{EFEFEF}}l l}
NL ES & 68.555 \\
ES NL & 68.954 \\
FR DE & 67.309 \\
DE FR & 67.802
\end{tabular}
\caption{AUC score of language pairs between language families (Romance and Germanic). In each row, first language is source and last language is destination.}
\label{table:auc_both}
\end{table*}

\begin{table*}[t]
\small
\centering
\begin{tabular}{lllllllllllll}
\rowcolor[HTML]{EFEFEF} 
 &
  \textbf{ES IT} &
  \textbf{ES FR} &
  \textbf{ES RO} &
  \textbf{IT ES} &
  \textbf{IT FR} &
  \textbf{IT RO} &
  \textbf{FR IT} &
  \textbf{FR ES} &
  \textbf{FR RO} &
  \textbf{RO ES} &
  \textbf{RO IT} &
  \textbf{RO FR} \\
\cellcolor[HTML]{EFEFEF}\textbf{0.2} & 16.21 & 19.45 & 10.82 & 17.12 & 19.45 & 15.7  & 15.32 & 16.67 & 10.13 & 14.02 & 11.2  & 23.81 \\
\cellcolor[HTML]{EFEFEF}\textbf{0.3} & 19.49 & 23.37 & 14.72 & 20.33 & 23.37 & 17.45 & 19.29 & 21.34 & 14.07 & 18.3  & 15.51 & 26.14 \\
\cellcolor[HTML]{EFEFEF}\textbf{0.4} & 20.82 & 25.33 & 16.07 & 22.74 & 25.33 & 18.73 & 20.72 & 23.12 & 15.96 & 20.3  & 17.4  & 27.92 \\
\cellcolor[HTML]{EFEFEF}\textbf{0.5} & 22.09 & 26.5  & 17.24 & 23.42 & 25.77 & 19.1  & 21.94 & 24.16 & 16.67 & 21.41 & 18.19 & 28.61 \\
\cellcolor[HTML]{EFEFEF}\textbf{0.6} & 22.1  & 27.39 & 17.6  & 23.69 & 26.82 & 19.14 & 22.64 & 24.55 & 17.45 & 22.34 & 19.02 & 29    \\
\cellcolor[HTML]{EFEFEF}\textbf{0.7} & 23.34 & 27.72 & 17.94 & 24.72 & 26.91 & 19.85 & 22.87 & 24.91 & 18    & 22.64 & 19.63 & 29.51 \\
\cellcolor[HTML]{EFEFEF}\textbf{0.8} & 23.48 & 28.56 & 18.72 & 24.88 & 27.77 & 19.67 & 22.92 & 25.59 & 18.59 & 23.51 & 20.18 & 29.89 \\
\cellcolor[HTML]{EFEFEF}\textbf{0.9} & 24.04 & 29.01 & 18.87 & 24.92 & 27.92 & 20.12 & 23.68 & 26.01 & 19.01 & 23.5  & 20.49 & 30.12 \\
\cellcolor[HTML]{EFEFEF}\textbf{1}   & 23.92 & 29.33 & 19.31 & 25.16 & 28.37 & 20.09 & 23.87 & 26.25 & 19.06 & 24.35 & 21.14 & 30.01 \\
\cellcolor[HTML]{EFEFEF}\textbf{Total Examples} &
  331236 &
  312182 &
  326634 &
  331196 &
  310982 &
  653202 &
  310942 &
  312134 &
  304960 &
  326630 &
  326592 &
  609974
\end{tabular}
\caption{The relative BLEU score as a function of the dataset size for the Romance languages. }
\label{table:romance1}
\end{table*}

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{fig2.jpeg}
\caption{Average performance of languages considered to be high or low intelligibility, out of the Romance language family. Performance is measured as the BLEU score evaluated on the test set of a model trained on a given subset for 50 epochs, divided by the BLEU score of a model trained on 100\% of the data.}
\label{fig:average_romance}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{fig3.jpeg}
\caption{Performance of two pairs of languages: Spanish-Romanian and Italian-Spanish. Italian Spanish is highly intelligible while Spanish Romanian is not. Performance is measured as the BLEU score evaluated on the test set of a model trained on a given subset for 50 epochs, divided by the BLEU score of a model trained on 100\% of the data. It can be seen that the intelligible pair scores better for smaller data sizes compared to the unintelligible pair.}
\label{fig:romance_cherry}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{fig3.jpeg}
\caption{Average relative BLEU results as a function of the data set size, split to the high and low mutual intelligibility in green and red respectively }
\label{fig:german_avg}
\end{figure}



\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{fig6.jpeg}
\caption{Performance of two pairs of languages: French-Spanish and Spanish-French to explore the a-symmetrical nature of mutual intelligibility. French - Spanish achieve a higher relative BLEU score consistently while also being more mutually intelligible. Performance is measured as the BLEU score evaluated on the test set of a model trained on a given subset for 50 epochs, divided by the BLEU score of a model trained on 100\% of the data. It can be seen that the intelligible pair scores better for smaller data sizes compared to the unintelligible pair.}
\label{fig:symmetry}
\end{figure}


\subsection{Germanic}

Considering the Germanic languages, most of the results must be looked at with a higher degree of skepticism, because of the inherent English exposure and the fact that English is the base for all language pairs, meaning each pair containing English as a source or target language was not pivoted. With this caveat in mind, table \ref{table:auc_germanic} shows the AUC scores for the Germanic language group. The correlation is even weaker (Pearson's r = -0.16, p-value=0.75).

Table \ref{table:germanic} shows the relative BLEU results. For clarity, we will not present the plot of all language pairs. Figure \ref{fig:german_avg} shows the average relative BLEU scores of the high and low intelligibility groups in the Germanic languages. Unlike the Romance, here we do not see a clear advantage to the high intelligibility pairs. A plausible explanation might be that high intelligibility pairs consist mainly of English, because it is measured by people who speak the language, unlike the NMT which does not have this prior knowledge. 


\begin{table}[t]
\small
\centering
\begin{tabular}{
>{\columncolor[HTML]{EFEFEF}}l l}
EN NL & 73.223 \\
\textbf{NL DE} & 72.875 \\
\textbf{DE EN} & 71.801 \\
\textbf{NL EN} & 73.578 \\
DE NL & 72.666 \\
EN DE & 72.826
\end{tabular}
\caption{AUC score per Germanic language pair. In each row, first language is source and last language is destination. Marked in bold are language pairs which are of high intelligibility.}
\label{table:auc_germanic}
\end{table}


\begin{table*}[t]
\small %
\centering
% \setlength{\tabcolsep}{4pt} %% default is 6pt
\begin{tabular}{
>{\columncolor[HTML]{EFEFEF}}l llllll}
\textbf{} &
  \cellcolor[HTML]{EFEFEF}\textbf{EN NL} &
  \cellcolor[HTML]{EFEFEF}\textbf{EN DE} &
  \cellcolor[HTML]{EFEFEF}\textbf{NL EN} &
  \cellcolor[HTML]{EFEFEF}\textbf{NL DE} &
  \cellcolor[HTML]{EFEFEF}\textbf{DE EN} &
  \cellcolor[HTML]{EFEFEF}\textbf{DE NL} \\
\textbf{0.2}            & 22.40  & 18.30  & 26.12  & 14.74  & 22.74  & 20.74  \\
\textbf{0.3}            & 26.47  & 22.20  & 30.11  & 18.60  & 26.37  & 22.84  \\
\textbf{0.4}            & 28.31  & 24.10  & 32.49  & 20.19  & 29.01  & 23.70  \\
\textbf{0.5}            & 29.14  & 25.00  & 34.24  & 21.23  & 30.07  & 24.12  \\
\textbf{0.6}            & 29.99  & 25.93  & 34.11  & 21.81  & 31.91  & 24.24  \\
\textbf{0.7}            & 30.09  & 26.05  & 34.88  & 21.84  & 32.10  & 24.44  \\
\textbf{0.8}            & 31.00  & 26.91  & 35.93  & 22.75  & 32.97  & 24.61  \\
\textbf{0.9}            & 31.50  & 27.52  & 36.52  & 23.07  & 33.39  & 24.70  \\
\textbf{100}            & 31.91  & 27.55  & 36.65  & 23.11  & 34.01  & 24.73  \\
\textbf{Total Examples} & 307180 & 320478 & 307180 & 291444 & 320478 & 583092
\end{tabular}%
\caption{BLEU results of the Germanic languages}
\label{table:germanic}
\end{table*}


\subsection{Cross Family}
We sampled two languages from each family: French and Spanish from Romance, German and Dutch from Germanic. We then trained a model for each cross family pair, which table \ref{table:auc_both} shows the AUC scores for. AUC scores for cross family translation is much lower, as the highest AUC score for cross family is 68.9 (ES-NL), with the lowest intra group AUC score being 69.9 (FR-RO), shown in table \ref{table:auc_romance}.


\subsection{Asymmetric intelligibility}

An interesting aspect of intelligibility is how a-symmetric it may be- this is very prominent in Table \ref{table:table1}, especially with the Romanian language; Romanian speakers can easily understand other Romance languages but not the other way around.
Figure \ref{fig:symmetry} shows this effect for the Italian and Spanish pair, as Italian-Spanish is more mutually intelligible than Spanish-Italian. It can be seen that Italian Spanish achieves a relative BLEU score of around 92\% on 40\% of the data, while Spanish-Italian requires 50\% to achieve similar results. 


==> links.tex <==
https://www.tandfonline.com/doi/full/10.1080/14790718.2017.1350185?scroll=top&needAccess=true - Mutual Intelligibility 
